Estimating Angle of Arrival (AoA) of multiple Echoes in a Steering Vector Space

Consider a microphone array, such as those present in Amazon Echos, conference phones, or self-driving cars. One of the goals of these arrays is to decode the angles in which acoustic signals arrive at them. This paper considers the problem of estimating K angle of arrivals (AoA), i.e., the direct path's AoA and the AoA of subsequent echoes. Significant progress has been made on this problem, however, solutions remain elusive when the source signal is unknown (such as human voice) and the channel is strongly correlated (such as in multipath settings). Today's algorithms reliably estimate the direct-path-AoA, but the subsequent AoAs diverge in noisy real-world conditions. We design SubAoA, an algorithm that improves on the current body of work. Our core idea models signal in a new AoA sub-space, and employs a cancellation approach that successively cancels each AoA to decode the next. We explain the behavior and complexity of the algorithm from the first principles, simulate the performance across a range of parameters, and present results from real-world experiments. Comparison against multiple existing algorithms like GCC-PHAT, MUSIC, and VoLoc shows increasing gains for the latter AoAs, while our computation complexity allows real-time operation. We believe progress in multi-AoA estimation is a fundamental building block to various acoustic and RF applications, including human or vehicle localization, multi-user separation, and even (blind) channel estimation.

==> fig/simu/backup.tex <==
%% backup tex for simulation section in Jan.24
\section{Simulation based Analysis}
In this section, we simulate the performance of \name\ to support the algorithm analysis above comparing with MUSIC.
We simulate the multipath in a $5$m by $5$m room with room impulse response generator from AudioLab ~\cite{RIR_gen,allen1979image}. 

\begin{figure*}[ht]
    \includegraphics[width=0.32\textwidth]{fig/simu/spec_w_0.pdf}
    \includegraphics[width=0.32\textwidth]{fig/simu/spec_v_0.pdf}
    \includegraphics[width=0.32\textwidth]{fig/simu/spec_v_10dB.pdf}

    \caption{AoA Likelihood where (a) white noise (b) speech as the signal in the noise-free environment, and (c) speech as the signal in a noisy (SNR=10dB) environment.}
    \label{fig:simu_spec}
    \minus
\end{figure*}

To confirm the robustness of \name\ against the noise, we simulate \name\ across different receiver position across the room using the speech signal of 0dB SNR.
Figure~\ref{fig:simu_music} presents the CDF of the $\theta_1$ and $\theta_2$

\begin{figure}[ht]
    \includegraphics[width=0.95\columnwidth]{fig/simu/cdf_music_0dB_simu.pdf}
    \minus
    \caption{Error compared with the MUSIC algorithm}
    \label{fig:simu_music}
    \minus
\end{figure}
% \vspace{1in}

\begin{figure}[ht]
    \includegraphics[width=0.425\columnwidth]{fig/simu/room_2.pdf}
    \includegraphics[width=0.54\columnwidth]{fig/simu/room_3.pdf}
    \minus
    \caption{Median error in a 5m by 5m room across different device locations.}
    \label{fig:simu_room}
    \minus
\end{figure}
% \vspace{1in}

\begin{figure}[ht]
    \includegraphics[width=0.45\columnwidth]{fig/simu/cdf_angdiff_2.pdf}
    \includegraphics[width=0.45\columnwidth]{fig/simu/cdf_angdiff_3.pdf}
    \minus
    \caption{Error for (a) $\theta_1$ and (b) $\theta_2$ in different path angular differences.}
    \label{fig:simu_ang_diff}
    \minus
\end{figure}
% \vspace{1in}

Figure ~\ref{fig:simu_spec} shows the AoA likelihood for each iteration. 
We put the receiver at $(1m,2m)$ and the speaker at $(2m,2m)$, 
. The ground truth AoAs are $\theta_{0:3}=[0^\circ,180^\circ,273\circ, 90^\circ]$, spanning the full AoA spectrum. 
$pk$ represents the likelihood of the $k-th iteration$, and the down triangle marks the ground truth $\theta_k$.
Note that $p0$ is also the MUSIC spectrum, as MUSIC only computes the noise space once and outputs the spectrum.

Figure ~\ref{fig:simu_spec}(a) and (b) compare the Gaussian signal with the recorded speech as the source. 
One can see that the source signal type does not affect the performance, although the order of $\theta_2$ and $\theta_3$ is reversed because these two paths are of comparable strength.
Interestingly, MUSIC also presents a nice spectrum of four peaks ($p0$) for human speech, a highly auto-correlated signal. 
This is because these four reflections are strong enough, such that the signal correlation between paths does not overwhelm the weak reflections.
However, because \name\ removes the estimated path component,
the peak for $p{1:3}$ is much higher than the corresponding peaks in $p0$, the MUSIC spectrum. 
The peak prominences ~\cite{prominence} are increased by $87\%$, $89\%$, and $100\%$ for $\theta_1$, $\theta_2$, and $\theta_3$ respectively. 
The latter path's gain is larger, because small echoes suffer from correlated source signals much in $p0$.

Figure ~\ref{fig:simu_spec}(c) presents the performance under the noisy environment. 
Once the noise kicks in, the small peaks in $p0$ disappear, and 
MUSIC fails to detect these small echoes, while \name\ could removes the estimated path one by one, and obtain a clear peak in each iteration.
\new
